Mastering Heterogeneous Behavioural Models

Heterogeneity is one important feature of complex systems, leading to the complexity of their construction and analysis. Moving the heterogeneity at model level helps in mastering the difficulty of composing heterogeneous models which constitute a large system. We propose a method made of an algebra and structure morphisms to deal with the interaction of behavioural models, provided that they are compatible. We prove that heterogeneous models can interact in a safe way, and therefore complex heterogeneous systems can be built and analysed incrementally. The Uppaal tool is targeted for experimentations.

==> extendedMealy.tex <==
% -*- coding: utf-8 -*- 

%--- Extended LTS = extended Mealy machine as a pivotal language for heterogeneous composition
\section{Multi-layered  Transition Systems}
\label{section:}

We define multi-layered transitions to handle the heterogeneity that appear in various behaviour models. The labels loosely integrate in severa layers the various aspects that come with the interacting models: 
data, guards, time constraints, communication statements, ...

Therefore a stack of facets is necessary.

\subsection{Composition of multi-layer labelled transition system}


\subsection{Filtering the layered transitions}
 



==> illustration.tex <==
\todo{Results and dicussion}



